Growth of Ultra-high Purity NaI(Tl) Crystal for Dark Matter Searches

The annual modulation of scintillation event rate observed by the DAMA/LIBRA experiment has been a long-standing controversy in the quest of the direct detection of dark matter. The effort to definitively confirm or refute the annual modulation has turned out to be challenging due to the lack of NaI(Tl) crystals with high enough radio-purity. Most recently, we successfully grew a 6-kg ingot free from contamination during growth, from which a 3.4-kg crystal scintillator was made. The $^{39}$K concentration in the final crystal is estimated to be 4.3$\pm$0.2~ppb, unprecedented for NaI(Tl) crystals. The $^{210}$Pb activity is estimated to be 0.34$\pm$0.04~mBq/kg via $\alpha$ counting of $^{210}$Po, among the lowest of currently-running NaI-based dark matter experiments except DAMA/LIBRA. More importantly, the techniques and protocols we have developed will further contribute to the growth of higher purity NaI(Tl) crystals for dark matter searches.

==> definitions.tex <==

%% LAYOUT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{geometry}
%\geometry{a4paper, total={6in, 8in}}
%%  for a4paper, total text area not exceeding 6in x 8in

%\geometry{legalpaper, landscape, margin=2in}
%% landscape orientation with all margin 2 in

\geometry{legalpaper, left=1in, right=0.75in, top=1in, bottom=1in}
%% individually control all margins


\usepackage{calc}
%% enable calculation of symbols like 1em


%% GRAPHS and TABLES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{graphicx}
\usepackage{subcaption}

\usepackage{booktabs}
\usepackage{colortbl}
    %% color cell in table
\usepackage{multirow}


%% MATH AND CHEMICAL SYMBOLS %%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{amsmath}
\usepackage[version=4]{mhchem}

\usepackage{xcolor}
    %%  black, blue, brown, cyan, darkgray, gray, green, lightgray, lime, magenta, olive, orange, pink, purple, red, teal, violet, white, yellow
    \definecolor{miku}{RGB}{64,224,208}
    %% model can be grey, rgb (0-1) or RGB (0-255)
    
\usepackage{url}



%\usepackage{natbib}


%% UNITS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\degreeC}{$^\circ$C}
\newcommand{\degC}{$^\circ$C}

\newcommand{\isotope}[2]{$^{\text{#2}}$#1}
\newcommand{\keVee}{keV$_{\text{ee}}$}
\newcommand{\inch}{$^{\prime\prime}$}
    %% inch
\newcommand{\minch}{^{\prime\prime}}
    %% inch symbol in math mode.

\newcommand{\noavail}{\text{n}\textbackslash{}\text{a}}
\newcommand{\na}{\noavail{}}
    % not available, i.k.a. n\a




==> graphs.tex <==
% Single Graph

% Note that linewidth refers to width of actual one line (columnwidth),
% while textwidth is the global width of text area.
% In two-column mode, linewidth is same or smaller than textwidth.

\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/color_wheel.png}
    \caption{Single figure.}
    \label{fig:color-info}
\end{figure}







% Subfigure
\begin{figure}[htb!]
    \centering
    \begin{subfigure}[t]{0.5\linewidth-1em}
    % em is the size of one M letter. -1em is used to compensate \quad parameter.
	    \centering
   	    \includegraphics[width=\linewidth]{figures/NaI_vapor_pressure_HT.png}
        \caption{Subfigure 1.}
        \label{fig:nai}
    \end{subfigure}
    \quad
    \begin{subfigure}[t]{0.5\linewidth-1em}
    	\centering
        \includegraphics[width=\linewidth]{figures/NaOH_vapor_pressure.png}
        \caption{Subfigure 2.}
        \label{fig:naoh}
    \end{subfigure}
	\caption{Subfigure/subcaption.}
    \label{fig:nai-naoh-vp}
\end{figure}

==> table.tex <==
%% Tips for making nice tables:

% * avoid vertical lines
% * avoid boxed cells - three horizontal lines are enough
% * when in doubt, align left


\iffalse
\begin{table}[htb!]
    \centering
    \caption{Simple table.}
    \label{tab:tab1}
    \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
    \ra{1.3}
    \begin{tabular}{*3c}
        \toprule
        \toprule
         & \ce{C10H12} & \ce{C10H8}\\
        \midrule
        MP & $-35.8$ & $80.3$\\
        BP & $206$-$208$ & $218$\\
        VP~(mbar) at $20$~\degreeC{} & $0.5$ & $0.125$\\
        \bottomrule
        \bottomrule
    \end{tabular}
\end{table}


%% table with adjusted row height and complex structure


\begin{table*}[htb!]
    \caption{\textcolor{red}{Table with stretched cell height and phantom column}}
    \label{tab:tab2}
    \centering
    \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
    \ra{1.3}
        %% this parameter controls vertical spacing of rows
        
    \begin{tabular}{@{}rclllcrrrc@{}}
        \toprule
        \toprule
&\phantom{a}& \multicolumn{3}{c}{A} & \phantom{abc}& \multicolumn{3}{c}{B}\\
\cmidrule{3-5} \cmidrule{7-9}
& & $t=0$ & $t=1$ & $t=2$ && $t=0$ & $t=1$ & $t=2$\\
Case 0\\
$c$ & & 1 & 2 & 3 && 4 & 5 & 6\\
$c$ & & 1 & 2 & 3 && 4 & 5 & 6\\
Case 1\\
$c$ & & 0.0357& 1.2473& 0.2119&& 0.3593& -0.2755& 2.1764\\
        \bottomrule
        \bottomrule
    \end{tabular}
\end{table*}



%% table with wrap text
% Table
\begin{table}[htbp]
    \centering
    \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
    \ra{1.3}
    \caption[]{Table with defined box width, text wrap, colored text and colored cell.}
    \label{tab:tab3}
    
    \begin{tabular}{@{}p{0.2\linewidth-2\arraycolsep} p{0.2\linewidth-2\arraycolsep} p{0.3\linewidth-2\arraycolsep} @{}}
    
        \toprule
        \toprule
        \textbf{Temperature} & \textbf{Duration} & \textbf{Characteristics} \\
        \midrule

$20$ \degreeC & $1$ & \textcolor{red}{Here is a very long text that might not fit within the specified width}\\[0.2em]
$120$ \degreeC & $1-3$ & \cellcolor{blue} \\[0.2em]
$240$ \degreeC & $1-2$ & \cellcolor{purple}\\[0.2em]
$320$ \degreeC & $1-2$ & \cellcolor{teal}\\[0.2em]
$380$ \degreeC & $1-2$ & \cellcolor{miku} \textcolor{blue}{Miku}\\[0.2em]

        \bottomrule
        \bottomrule
    \end{tabular}
\end{table}
\fi
